Ensemble Squared: A Meta AutoML System

There are currently many barriers that prevent non-experts from exploiting machine learning solutions ranging from the lack of intuition on statistical learning techniques to the trickiness of hyperparameter tuning. Such barriers have led to an explosion of interest in automated machine learning (AutoML), whereby an off-the-shelf system can take care of many of the steps for end-users without the need for expertise in machine learning. This paper presents Ensemble Squared (Ensemble$^2$), an AutoML system that ensembles the results of state-of-the-art open-source AutoML systems. Ensemble$^2$ exploits the diversity of existing AutoML systems by leveraging the differences in their model search space and heuristics. Empirically, we show that diversity of each AutoML system is sufficient to justify ensembling at the AutoML system level. In demonstrating this, we also establish new state-of-the-art AutoML results on the OpenML tabular classification benchmark.

==> tableall.tex <==
{
\renewcommand{\arraystretch}{1.25}
\begin{table*}[tbph]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c||cccccc|c|c}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}OpenML \\ Dataset ID \\ \end{tabular}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}AlphaD3M \\ \end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Axolotl \\ \end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}CMU AutoML \\ \end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}AutoGluon \\  \end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Auto-Sklearn \\ \end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Auto-Sklearn-$2$ \\ \end{tabular}}} &
  \multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ensemble$^2$ \\ \end{tabular}}} \\ \hline
2          & 0.600 $\pm$ 0.000 & 0.981 $\pm$ 0.000 & 0.822 $\pm$ 0.000 & \textbf{0.990 $\pm$ 0.001} & 0.985 $\pm$ 0.003 & 0.976 $\pm$ 0.007 & 0.982 $\pm$ 0.003    \\
3          & 0.515 $\pm$ 0.002 & 0.990 $\pm$ 0.001 & \textbf{0.996 $\pm$ 0.000} & 0.993 $\pm$ 0.002 & 0.654 $\pm$ 0.463 & 0.995 $\pm$ 0.002 & 0.994 $\pm$ 0.002    \\
5          & 0.357 $\pm$ 0.011 & \textbf{0.744 $\pm$ 0.005} & 0.475 $\pm$ 0.000 & 0.683 $\pm$ 0.005 & 0.724 $\pm$ 0.016 & 0.479 $\pm$ 0.339 & 0.705 $\pm$ 0.011    \\
12         & 0.092 $\pm$ 0.003 & 0.937 $\pm$ 0.005 & 0.207 $\pm$ 0.000 & 0.973 $\pm$ 0.001 & 0.651 $\pm$ 0.460 & 0.974 $\pm$ 0.001 & \textbf{0.974 $\pm$ 0.001}    \\
31         & 0.670 $\pm$ 0.025 & 0.726 $\pm$ 0.002 & 0.745 $\pm$ 0.000 & \textbf{0.783 $\pm$ 0.001} & 0.756 $\pm$ 0.017 & \textbf{0.783 $\pm$ 0.002} & 0.775 $\pm$ 0.002    \\
54         & 0.293 $\pm$ 0.011 & 0.743 $\pm$ 0.013 & 0.768 $\pm$ 0.001 & \textbf{0.841 $\pm$ 0.010} & 0.797 $\pm$ 0.016 & 0.754 $\pm$ 0.018 & 0.834 $\pm$ 0.012    \\
1067       & 0.767 $\pm$ 0.036 & 0.813 $\pm$ 0.032 & 0.845 $\pm$ 0.000 & 0.857 $\pm$ 0.002 & 0.857 $\pm$ 0.004 & 0.848 $\pm$ 0.006 & \textbf{0.860 $\pm$ 0.001}    \\
1111       & 0.655 $\pm$ 0.463 & 0.964 $\pm$ 0.024 & \textbf{0.983 $\pm$ 0.000} & \textbf{0.983 $\pm$ 0.000} & \textbf{0.983 $\pm$ 0.000} & \textbf{0.983 $\pm$ 0.000} & \textbf{0.983 $\pm$ 0.000}    \\
1169       & 0.339 $\pm$ 0.240 & -             & 0.650 $\pm$ 0.000 & 0.661 $\pm$ 0.005 & 0.438 $\pm$ 0.309 & \textbf{0.666 $\pm$ 0.001} & 0.662 $\pm$ 0.005    \\
1461       & 0.843 $\pm$ 0.005 & 0.893 $\pm$ 0.007 & 0.903 $\pm$ 0.000 & \textbf{0.909 $\pm$ 0.000} & 0.904 $\pm$ 0.001 & 0.906 $\pm$ 0.001 & 0.908 $\pm$ 0.000    \\
1464       & 0.723 $\pm$ 0.009 & 0.747 $\pm$ 0.000 & 0.743 $\pm$ 0.000 & 0.750 $\pm$ 0.007 & 0.753 $\pm$ 0.018 & 0.760 $\pm$ 0.024 & \textbf{0.768 $\pm$ 0.022}    \\
1468       & -             & 0.927 $\pm$ 0.009 & 0.937 $\pm$ 0.002 & 0.914 $\pm$ 0.006 & 0.924 $\pm$ 0.004 & \textbf{0.941 $\pm$ 0.007} & 0.938 $\pm$ 0.004    \\
1486       & 0.395 $\pm$ 0.279 & 0.966 $\pm$ 0.003 & 0.970 $\pm$ 0.001 & \textbf{0.973 $\pm$ 0.001} & 0.966 $\pm$ 0.002 & 0.648 $\pm$ 0.458 & \textbf{0.973 $\pm$ 0.001}    \\
1489       & 0.584 $\pm$ 0.001 & 0.890 $\pm$ 0.000 & 0.901 $\pm$ 0.000 & \textbf{0.902 $\pm$ 0.002} & 0.886 $\pm$ 0.005 & 0.890 $\pm$ 0.001 & \textbf{0.902 $\pm$ 0.002}    \\
1590       & 0.434 $\pm$ 0.307 & 0.856 $\pm$ 0.002 & 0.860 $\pm$ 0.000 & \textbf{0.876 $\pm$ 0.000} & 0.873 $\pm$ 0.001 & 0.864 $\pm$ 0.012 & \textbf{0.876 $\pm$ 0.000}    \\
1596       & 0.255 $\pm$ 0.180 & -             & 0.650 $\pm$ 0.035 & 0.880 $\pm$ 0.006 & 0.317 $\pm$ 0.448 & \textbf{0.955 $\pm$ 0.000} & 0.925 $\pm$ 0.021    \\
4135       & 0.607 $\pm$ 0.429 & 0.946 $\pm$ 0.001 & 0.947 $\pm$ 0.000 & \textbf{0.949 $\pm$ 0.000} & 0.629 $\pm$ 0.445 & 0.947 $\pm$ 0.001 & \textbf{0.949 $\pm$ 0.000}    \\
23512      & 0.337 $\pm$ 0.238 & 0.447 $\pm$ 0.317 & 0.719 $\pm$ 0.000 & 0.484 $\pm$ 0.342 & 0.483 $\pm$ 0.342 & \textbf{0.727 $\pm$ 0.002} & 0.725 $\pm$ 0.003    \\
23517      & 0.503 $\pm$ 0.000 & 0.518 $\pm$ 0.001 & 0.519 $\pm$ 0.000 & 0.511 $\pm$ 0.005 & 0.519 $\pm$ 0.001 & \textbf{0.520 $\pm$ 0.001} & 0.517 $\pm$ 0.002    \\
40668      & 0.439 $\pm$ 0.310 & 0.704 $\pm$ 0.071 & 0.836 $\pm$ 0.003 & 0.837 $\pm$ 0.005 & 0.840 $\pm$ 0.002 & \textbf{0.850 $\pm$ 0.002} & 0.846 $\pm$ 0.002    \\
40685      & 0.431 $\pm$ 0.305 & \textbf{1.000 $\pm$ 0.000} & \textbf{1.000 $\pm$ 0.000} & \textbf{1.000 $\pm$ 0.000} & 0.789 $\pm$ 0.000 & 0.997 $\pm$ 0.000 & \textbf{1.000 $\pm$ 0.000}    \\
40975      & 0.614 $\pm$ 0.057 & 0.973 $\pm$ 0.000 & 0.969 $\pm$ 0.003 & \textbf{0.979 $\pm$ 0.001} & 0.643 $\pm$ 0.455 & 0.977 $\pm$ 0.006 & \textbf{0.979 $\pm$ 0.001}    \\
40981      & 0.523 $\pm$ 0.007 & 0.862 $\pm$ 0.000 & 0.841 $\pm$ 0.000 & 0.864 $\pm$ 0.007 & 0.586 $\pm$ 0.414 & \textbf{0.874 $\pm$ 0.013} & 0.867 $\pm$ 0.010    \\
40984      & 0.149 $\pm$ 0.003 & 0.924 $\pm$ 0.001 & 0.939 $\pm$ 0.000 & \textbf{0.940 $\pm$ 0.001} & 0.918 $\pm$ 0.001 & 0.929 $\pm$ 0.002 & 0.939 $\pm$ 0.001    \\
40996      & 0.066 $\pm$ 0.047 & -             & 0.501 $\pm$ 0.142 & \textbf{0.896 $\pm$ 0.001} & -             & -             & \textbf{0.896 $\pm$ 0.001}    \\
41027      & 0.343 $\pm$ 0.242 & 0.867 $\pm$ 0.005 & 0.874 $\pm$ 0.000 & \textbf{0.962 $\pm$ 0.002} & 0.883 $\pm$ 0.005 & 0.866 $\pm$ 0.002 & \textbf{0.962 $\pm$ 0.002}    \\
41138      & 0.643 $\pm$ 0.455 & 0.662 $\pm$ 0.455 & 0.993 $\pm$ 0.000 & \textbf{0.994 $\pm$ 0.000} & 0.992 $\pm$ 0.000 & 0.993 $\pm$ 0.000 & 0.993 $\pm$ 0.000    \\
41142      & -             & -             & 0.708 $\pm$ 0.009 & \textbf{0.735 $\pm$ 0.003} & 0.726 $\pm$ 0.004 & 0.725 $\pm$ 0.002 & \textbf{0.735 $\pm$ 0.003}    \\
41143      & 0.477 $\pm$ 0.001 & 0.800 $\pm$ 0.000 & 0.800 $\pm$ 0.002 & 0.805 $\pm$ 0.003 & 0.801 $\pm$ 0.002 & 0.267 $\pm$ 0.378 & \textbf{0.806 $\pm$ 0.003}    \\
41146      & 0.351 $\pm$ 0.248 & 0.934 $\pm$ 0.000 & \textbf{0.955 $\pm$ 0.000} & 0.948 $\pm$ 0.001 & 0.939 $\pm$ 0.005 & 0.934 $\pm$ 0.003 & 0.949 $\pm$ 0.001    \\
41147      & 0.333 $\pm$ 0.236 & -             & 0.645 $\pm$ 0.007 & -             & 0.682 $\pm$ 0.001 & \textbf{0.684 $\pm$ 0.001} & 0.683 $\pm$ 0.001    \\
41150      & 0.605 $\pm$ 0.000 & 0.542 $\pm$ 0.385 & 0.940 $\pm$ 0.000 & 0.946 $\pm$ 0.001 & 0.939 $\pm$ 0.000 & 0.945 $\pm$ 0.002 & \textbf{0.947 $\pm$ 0.001}    \\
41159      & -             & -             & -             & \textbf{0.821 $\pm$ 0.003} & -             & -             & 0.819 $\pm$ 0.001    \\
41161      & -             & -             & -             & \textbf{0.997 $\pm$ 0.001} & -             & -             & \textbf{0.997 $\pm$ 0.001}    \\
41163      & -             & -             & 0.488 $\pm$ 0.122 & \textbf{0.989 $\pm$ 0.000} & 0.975 $\pm$ 0.002 & 0.932 $\pm$ 0.003 & 0.985 $\pm$ 0.003    \\
41164      & 0.186 $\pm$ 0.001 & 0.287 $\pm$ 0.035 & 0.188 $\pm$ 0.000 & \textbf{0.721 $\pm$ 0.003} & 0.679 $\pm$ 0.006 & 0.656 $\pm$ 0.012 & \textbf{0.721 $\pm$ 0.003}    \\
41165      & -             & -             & -             & \textbf{0.493 $\pm$ 0.005} & -             & -             & 0.486 $\pm$ 0.010    \\
41166      & 0.109 $\pm$ 0.077 & 0.373 $\pm$ 0.150 & 0.611 $\pm$ 0.060 & \textbf{0.713 $\pm$ 0.003} & 0.682 $\pm$ 0.005 & 0.654 $\pm$ 0.001 & 0.707 $\pm$ 0.006    \\
41167      & 0.003 $\pm$ 0.000 & -             & 0.583 $\pm$ 0.027 & \textbf{0.909 $\pm$ 0.001} & 0.684 $\pm$ 0.001 & 0.503 $\pm$ 0.356 & \textbf{0.909 $\pm$ 0.001}    \\
41168      & 0.248 $\pm$ 0.175 & 0.576 $\pm$ 0.149 & 0.679 $\pm$ 0.027 & \textbf{0.719 $\pm$ 0.002} & 0.704 $\pm$ 0.002 & 0.713 $\pm$ 0.001 & 0.718 $\pm$ 0.003    \\
41169      & 0.026 $\pm$ 0.000 & 0.310 $\pm$ 0.012 & 0.350 $\pm$ 0.014 & 0.394 $\pm$ 0.000 & 0.296 $\pm$ 0.001 & 0.332 $\pm$ 0.003 & \textbf{0.395 $\pm$ 0.001}\\ \hline
{\begin{tabular}[c]{@{}c@{}}Average Accuracy\\ (across datasets)\\ \end{tabular}}                               & 0.354 & 0.583 & 0.696 & 0.819 & 0.679 & 0.718 & \textbf{0.845}\\ \hline
{\begin{tabular}[c]{@{}c@{}}Average Rank\\ (out of 7)\\ \end{tabular}}                               & 5.683 & 4.415 & 3.488 & 2.024 & 3.439 & 2.756 & \textbf{1.659}\\ \hline
\end{tabular}%
}
\caption{Comparison between Ensemble$^2$ and SOTA AutoML systems. All systems were run for one hour each. Ensemble$^2$ uses an ensemble of size three. The highest accuracy achieved by a method on a dataset is shown in boldface and dash ($-$) shows a method failed to produce outputs for a dataset.}
\label{tab:sota}
\end{table*}
}

==> tableid2name.tex <==
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 OpenML Dataset ID & OpenML Dataset Name \\
 \hline
 2 & anneal \\ 
 3 & kr-vs-kp  \\
 5 & arrhythmia \\
 12 & mfeat-factors \\
 31 & credit-g \\
 54 & vehicle \\
 1067 & kc1 \\
 1111 & KDDCup09\_appetency  \\
 1169 & airlines   \\
 1461 & bank-marketing \\
 1464 & blood-transfusion-service-center  \\
 1468 & cnae-9 \\
 1486 & nomao \\
 1489 & phoneme \\
 1590 & adult \\
 1596 & covertype \\
 4135 & Amazon\_employee\_access \\
 23512 & higgs \\
 23517 & numerai$28.6$  \\
 40668 & connect-4 \\
 40685 & shuttle \\
 40975 & car \\
 40981 & Australian \\
 40984 & segment \\
 40996 & Fashion-MNIST \\
 41027 & jungle\_chess\_2pcs\_raw\_endgame\_complete \\
 41138 & APSFailure \\
 41142 & christine \\
 41143 & jasmine \\
 41146 & sylvine \\
 41147 & albert \\
 41150 & MiniBooNE \\
 41159 & guillermo \\
 41161 & riccardo \\
 41163 & dilbert \\
 41164 & fabert \\
 41165 & robert \\
 41166 & volkert \\
 41167 & dionis \\
 41168 & jannis \\
 41169 & helena \\
 \hline
\end{tabular}
\end{center}

